On Symbolic Approaches for Computing the Matrix Permanent

Counting the number of perfect matchings in bipartite graphs, or equivalently computing the permanent of 0-1 matrices, is an important combinatorial problem that has been extensively studied by theoreticians and practitioners alike. The permanent is #P-Complete; hence it is unlikely that a polynomial-time algorithm exists for the problem. Researchers have therefore focused on finding tractable subclasses of matrices for permanent computation. One such subclass that has received much attention is that of sparse matrices i.e. matrices with few entries set to 1, the rest being 0. For this subclass, improved theoretical upper bounds and practically efficient algorithms have been developed. In this paper, we ask whether it is possible to go beyond sparse matrices in our quest for developing scalable techniques for the permanent, and answer this question affirmatively. Our key insight is to represent permanent computation symbolically using Algebraic Decision Diagrams (ADDs). ADD-based techniques naturally use dynamic programming, and hence avoid redundant computation through memoization. This permits exploiting the hidden structure in a large class of matrices that have so far remained beyond the reach of permanent computation techniques. The availability of sophisticated libraries implementing ADDs also makes the task of engineering practical solutions relatively straightforward. While a complete characterization of matrices admitting a compact ADD representation remains open, we provide strong experimental evidence of the effectiveness of our approach for computing the permanent, not just for sparse matrices, but also for dense matrices and for matrices with "similar" rows.

==> proof.tex <==
\section{Tractability}
\begin{lemma}
	The size of Row Product ADD  of a 0-1 $ n \times n $ matrix $ \mat{A} $ with corresponding bipartite graph $ G_{\mat{A}} $ is bounded by $ \mathcal{O}(n2^q) $ where $ q $ is the primal pathwidth of $ G_{\mat{A}} $
\end{lemma}

\begin{proof}
	This proof largely follows the one given in Ferrara et al. for OBDDs of bounded pathwidth CNF formulas.
	
	Let the Primal path decomposition of $ \mat{A} $ be $(P,L)$. Assume without loss of generality that $P=\{1,...,k\}$. We construct a variable order from the path decomposition as follows: Define $First(x) = min({p\in P|v \in L(p)})$ and $Last(x) = max({p\in P|v\in L(p)})$. Now sort the variables in increasing lexicographic order according to $(First(x),Last(x))$; that is, define the variable order so that if $x < y$, then either $First(x)< First(y)$ or $First(x)=First(y)$ and $Last(x)< Last(y)$. We show that,  using  this  variable order, there  are  at  most $2^q$ nodes per  level.  The  claim  then follows. 
	
	For each row $r$, we define $min(r)$ as the index of the lowest ordered variable in $r$ and correspondingly for $max(r)$.  Consider level $i$ of the ADD, corresponding to the variable $x_i$. The row set $R$ can be partitioned into three classes with respect to level $i$, $R_{ended}={r|max(r)< i}$, $R_{cur}={r|min(r)\le i <max(r)}$, and $R_{untouched}={r|i <min(r)}$. 
	
	A node $u$ at level $i$ corresponds to a set $A_u$ of partial assignments to variables, where each partial assignment $a\in A_u$ is an element in $2^{x_1...x_{i-1}}$. From the  semantics  of  ADDs,  we  know that all partial assignments $a$ in $A_u$ are  equivalent with  respect to  extensions,  i.e., given $a' \in 2^\{x_i,...,x_n\}$ and $a\in A_u$,  we  have  that $ a \cup a' \models R$ iff  for  every $a'' \in A_u$, $a''\cup a'\models R$. If for $a \in A_u$, $a\not \models R_{ended}$, then we know that for every extension $a\cup a'$ of $a$ we have that $a\cup a'\not\models R_{ended}$, so $a\cup a'\not\models R$. Thus, the node $u$ is identical to Boolean 0 and should not exist at level $i$. It follows that for every $a\in A_u$, $a\models R_{ended}$. We also know that all rows in $R_{untouched}$ have none of their variables assigned by $a\in A_u$.
	
	Each partial assignment $a$ at level $i$ can be associated with a subset $M_a\subseteq R_{cur} $ where $M_a={r|r\in R_{cur},a\models r}$, i.e., the clauses in $R_{cur}$ that are already satisfied by $a$ before reading the variable $x_i$. We know that none of the clauses in $R_{cur}$ have failed (all literals assigned to false) so far, since by definition of $R_{cur}$ all such clauses have literals with variables beyond $x_{i-1}$. Suppose that for two distinct nodes $u$ and $v$ at level $i$ there exists $a_u\in A_u$ and $a_v\in A_v$ such that $M_{a_u} = M_{a_v}$. Since $u$ and $v$ are distinct, there is a partial assignment $a\in 2^\{x_i,...,x_n\}$ that distinguishes between $u$ and $v$; say, $a_u\cup a\models R$ and $a_v \cup a\not\models R$. Since $a_u$ and $a_v$, however, both satisfy $R_{ended}$, both are undefined on the variables of $R_{untouched}$, and we also have, by assumption, that $M_{a_u}=M_{a_v}$, we must have that $a_u\cup a\models R$ iff $a_v\cup a\models R$ - a contradiction. It follows that $M_{a_u}\not = M_{a_v}$.
	
	Let $j=First(x_i)$. We know that $L(j)$ contains at most $q+ 1$ variables, including $ x_i$. Let $Var_i=L(j)\cap\{x_1,...,x_{i-1}\}$, then $Var_i$ has at most $q$ variables. Suppose that $u$ and $v$ are two nodes at level $i$ such that there exists $a_u\in A_u$ and $a_v\in A_v$ where $a_u$ and $a_v$ agree on $Var_i$. We show then $M_{a_u}=M_{a_v}$. Consider a row $r\in R_{cur}$. We know that all the variables of $r$ occur in $L(k)$ for some $k$. We cannot have $k < j$, since then we’d have $r\in R_{ended}$, so $k\ge j$. If $x_h$ occurs in $r$ for some $h < i$, then by construction $x_h\in L(j')$ for some $j'\le j$. By the property of path decompositions it follows that $x_h\in L(j)$. Since $a_u$ and $a_v$ agree on $Var_i$, it follows that they agree on $r$. We showed that if $u$ and $v$ are distinct, then for every $a_u \in A_u$ and $a_v\in A_v$, $M_{a_u}\not=M_{a_v}$. It follows that $a_u$ and $a_v$ cannot agree on $Var_i$. Since $Var_i$ has at most $q$ variables, there can be at most $2^q$ nodes at level $i$. The claim follows since the OBDD has $n$ levels.
\end{proof}
